Beware the evolving 'intelligent' web service! An integration architecture tactic to guard AI-first components

Intelligent services provide the power of AI to developers via simple RESTful API endpoints, abstracting away many complexities of machine learning. However, most of these intelligent services-such as computer vision-continually learn with time. When the internals within the abstracted 'black box' become hidden and evolve, pitfalls emerge in the robustness of applications that depend on these evolving services. Without adapting the way developers plan and construct projects reliant on intelligent services, significant gaps and risks result in both project planning and development. Therefore, how can software engineers best mitigate software evolution risk moving forward, thereby ensuring that their own applications maintain quality? Our proposal is an architectural tactic designed to improve intelligent service-dependent software robustness. The tactic involves creating an application-specific benchmark dataset baselined against an intelligent service, enabling evolutionary behaviour changes to be mitigated. A technical evaluation of our implementation of this architecture demonstrates how the tactic can identify 1,054 cases of substantial confidence evolution and 2,461 cases of substantial changes to response label sets using a dataset consisting of 331 images that evolve when sent to a service.

==> frontmatter.tex <==
\title[An integration architecture tactic to guard AI-first components]{Beware the evolving `intelligent' web service!\\An integration architecture tactic to guard AI-first components}

%

\author{Alex Cummaudo}
\email{ca@deakin.edu.au}
\orcid{0000-0001-7878-6283}
\affiliation{%
\department{Applied Artificial Intelligence Inst.}
\institution{Deakin University}
\city{Geelong}
\country{Australia}
}

\author{Scott Barnett}
\email{scott.barnett@deakin.edu.au}
\orcid{0000-0002-3187-4937}
\affiliation{%
\department{Applied Artificial Intelligence Inst.}
\institution{Deakin University}
\city{Geelong}
\country{Australia}
}

\author{Rajesh Vasa}
\email{rajesh.vasa@deakin.edu.au}
\orcid{0000-0003-4805-1467}
\affiliation{%
\department{AApplied Artificial Intelligence Inst.}
\institution{Deakin University}
\city{Geelong}
\country{Australia}
}

\author{John Grundy}
\email{john.grundy@monash.edu}
\orcid{0000-0003-4928-7076}
\affiliation{%
\department{Faculty of Information Technology}
\institution{Monash University}
\city{Clayton}
\country{Australia}
}

\author{Mohamed Abdelrazek}
\email{mohamed.abdelrazek@deakin.edu.au}
\orcid{0000-0003-3812-9785}
\affiliation{%
\department{School of Information Technology}
\institution{Deakin University}
\city{Geelong}
\country{Australia}
}

\begin{abstract}
%
Intelligent services provide the power of AI to developers via simple RESTful API endpoints, abstracting away many complexities of machine learning.
%
However, most of these intelligent services---such as computer vision---continually learn with time.
%
%
When the internals within the abstracted `black box' become hidden and evolve, pitfalls emerge in the robustness of applications that depend on these evolving services. 
Without adapting the way developers plan and construct projects reliant on intelligent services, significant gaps and risks result in both project planning and development.
Therefore, how can software engineers best mitigate software evolution risk moving forward, thereby ensuring that their own applications maintain quality?
%
%
Our proposal is an architectural tactic designed to improve intelligent service-dependent software robustness. The tactic involves creating an application-specific benchmark dataset baselined against an intelligent service, enabling evolutionary behaviour changes to be mitigated. 
%
A technical evaluation of our implementation of this architecture demonstrates how the tactic can identify 1,054 cases of substantial confidence evolution and 2,461 cases of substantial changes to response label sets using a dataset consisting of 331 images that evolve when sent to a service.
\end{abstract}

\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10002951.10003260.10003304</concept_id>
<concept_desc>Information systems~Web services</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10011007.10011074.10011111.10011113</concept_id>
<concept_desc>Software and its engineering~Software evolution</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10010583.10010750.10010751.10010752</concept_id>
<concept_desc>Hardware~Error detection and error correction</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010520.10010521.10010537.10010538</concept_id>
<concept_desc>Computer systems organization~Client-server architectures</concept_desc>
<concept_significance>100</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Information systems~Web services}
\ccsdesc[500]{Software and its engineering~Software evolution}
\ccsdesc[300]{Hardware~Error detection and error correction}
\ccsdesc[100]{Computer systems organization~Client-server architectures}

\keywords{intelligent web services, software architecture, software evolution}

\renewcommand{\shortauthors}{Alex Cummaudo et al.}

\acmConference[ESEC/FSE 2020]{The 28th ACM Joint European Software Engineering Conference and Symposium on the Foundations of Software Engineering}{8 - 13 November, 2020}{Sacramento, California, United States}


==> preamble/extended.tex <==
\input{extended/authblk}
\input{extended/bibliography}
\input{extended/extra}
\input{extended/footnotes}
\input{extended/graphics}
\input{extended/listings}
\input{extended/tables}
\input{extended/todo}

==> preamble/extended/authblk.tex <==
% \usepackage{authblk}
% \renewcommand*{\Authsep}{, }
% \renewcommand*{\Authand}{, }
% \renewcommand*{\Authands}{, }
% \renewcommand*{\Affilfont}{\normalsize\normalfont}

==> preamble/extended/bibliography.tex <==
\usepackage{natbib}
\bibliographystyle{ACM-Reference-Format}


==> preamble/extended/footnotes.tex <==
\usepackage[multiple]{footmisc} % Two footnotes at the one point

\newcommand{\footnoteurl}[2]{\footnote{{#1} last accessed #2.}} % URL-cited footnotes

==> preamble/extended/graphics.tex <==
\usepackage{graphicx}
\graphicspath{{images/}{../images/}}


==> preamble/extended/listings.tex <==
\usepackage{listings}
\usepackage{textcomp}
\usepackage{color}
\definecolor{maroon}{rgb}{0.5,0,0}
\definecolor{darkgreen}{rgb}{0,0.5,0}

\renewcommand{\lstlistlistingname}{List of Listings}

\lstset{%
    % Basic design
    basicstyle={\footnotesize\ttfamily\color{black}},
    captionpos=t,
    abovecaptionskip=.5\baselineskip,
    belowcaptionskip=.5\baselineskip,
    columns=fullflexible,
    showstringspaces=false,
    commentstyle=\color{gray}\upshape,
    frame=none,
    upquote=true,
    % Line numbers
    xleftmargin={0.75cm},
    numbers=left,
    stepnumber=1,
    firstnumber=1,
    numberfirstline=true,
    stringstyle=\color{blue},
    %identifierstyle=\color{maroon},
    commentstyle=\color{darkgreen},
    keywordstyle=\color{red},
    upquote=true,
    breaklines=true,
    postbreak=\mbox{\textcolor{red}{$\hookrightarrow$}\space},
    literate={±}{{$\pm$}}1,
    escapeinside={(*}{*)}
}


\newcommand{\beginlstdelim}[3]
{%
  \def\endlstdelim{#2\egroup}%
  \ttfamily#1\bgroup\color{#3}\aftergroup\endlstdelim%
}

\lstdefinestyle{xml_style}
{
  morestring=[b]",
  moredelim=*[s][\bfseries\color{maroon}]{<}{>},
  moredelim=*[s][\bfseries\color{maroon}]{</}{>},
  morecomment=[s]{<?}{?>},
  morecomment=[s]{<!--}{-->},
}

\lstdefinestyle{json_style}
{
  morestring=[b]",
  comment=[l]{//},
  keywordstyle=\bfseries\color{maroon}
}

\lstdefinelanguage{JSON}
{
  style=json_style
}

\lstdefinelanguage{XML}
{
  style=xml_style
}


==> preamble/extended/tables.tex <==
% Use booktabs
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{makecell}
\newcommand{\tablefit}[1]{\resizebox{\linewidth}{!}{#1}}
\newcommand{\tablefitlandscape}[1]{\resizebox{1.2\paperwidth}{!}{#1}}


==> preamble/extended/todo.tex <==
\usepackage{xcolor}
\newcommand{\todo}[2][]{{\color{red} \slshape $\langle$~\textsc{\small\underline{todo}}: \textbf{#2}~{\color{darkgray}\textit{#1}}$\rangle$}}
%\newcommand{\todo}[2][]{#1}
\newcommand{\tonote}[1]{\textbf{\sffamily\footnotesize[#1]}}
\newcommand{\tocite}[1]{\tonote{cite:{#1}}}
\newcommand{\comnum}[1]{(Comment\##1)}

==> preamble/simple.tex <==
\usepackage{hyperref}
\input{simple/author}
\input{simple/captions}
\input{simple/cleverref}
\input{simple/geometry}
\input{simple/graphics}
\input{simple/typesetting}

==> preamble/simple/author.tex <==
\author{Alex Cummaudo\\Applied Artificial Intelligence Institute\\Deakin University, Australia}
\date{\today}


==> preamble/simple/captions.tex <==
\usepackage[labelfont=bf]{caption}

==> preamble/simple/cleverref.tex <==
\usepackage[capitalise,noabbrev,nameinlink]{cleveref}
\Crefname{lstlisting}{Listing}{Listings}

==> preamble/simple/geometry.tex <==
\usepackage{geometry}
\newgeometry{top=2.25cm,right=2cm,bottom=2.5cm,left=3cm}


==> preamble/simple/graphics.tex <==
\usepackage{graphicx}
\graphicspath{{images/}{../images/}}


==> preamble/simple/typesetting.tex <==
% Linespread of 1.5 as required by SIT
\linespread{1.5}
% Times new roman package
\usepackage{mathptmx}
% Change font style for sub-sub section
\usepackage{sectsty}
\subsubsectionfont{\normalfont\itshape}
